The Cost of Skeletal Call-by-Need, Smoothly

Skeletal call-by-need is an optimization of call-by-need evaluation also known as "fully lazy sharing": when the duplication of a value has to take place, it is first split into "skeleton", which is then duplicated, and "flesh" which is instead kept shared. Here, we provide two cost analyses of skeletal call-by-need. Firstly, we provide a family of terms showing that skeletal call-by-need can be asymptotically exponentially faster than call-by-need in both time and space; it is the first such evidence, to our knowledge. Secondly, we prove that skeletal call-by-need can be implemented efficiently, that is, with bi-linear overhead. This result is obtained by providing a new smooth presentation of ideas by Shivers and Wand for the reconstruction of skeletons, which is then smoothly plugged into the study of an abstract machine following the distillation technique by Accattoli et al.

==> figures/figure-cbneed-machine.tex <==
% !TEX root = ../main.tex
\begin{figure}[t!]
\centering
\fbox{
$\begin{array}{c}
\begin{array}{r@{\hspace{.25cm}} rcl  @{\hspace{.5cm}}  @{\hspace{.5cm}} r @{\hspace{.25cm}} rcl}
	\textsc{Stacks} & \stack 	& \grameq & \stempty \mid \tm \cons \stack
	&
	\textsc{Chains} &	\chain	& \grameq & \stempty \mid \chain\cons(\var, \stack, \genv)
	\\
	\textsc{States} &	\state	& \defeq & \glamst\chain\tm\stack\genv
	&
	\textsc{Environments} & \genv	& \grameq & \stempty \mid \esub\var\tm \cons \genv 

\end{array}
\\
\hline

\textsc{Transitions}
\\
  	{\setlength{\arraycolsep}{0.35em}
  	\begin{array}{c|c|c|c||l||c|c|c|cccc}
		 \mbox{Chain} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} 
		&&
		 \mbox{Chain} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} \\
\hhline{=|=|=|=|=|=|=|=|=}
		 \chain & \tm\tmtwo & \stack &  \genv
	  	&\tomachseaone&
	  	 \chain & \tm & \tmtwo\cons\stack & \genv
	  	\\
%\hhline{-|-|-|---|-|-|-}
%
		 \chain & \la\var\tm & \tmtwo \cons\stack  &\genv
		& \tomachbeta &
		\chain &  \tm & \stack  &\esub\var\tmtwo\cons\genv
		\\
		
		 \chain & \var & \stack & \genv\cons\esub\var\tm\cons\genvtwo
	  	&\tomachseatwo &
		 \chain\cons(\var, \stack, \genv) & \tm & \stempty & \genvtwo 
		 & \text{if } \tm\neq\val
	  	\\
		
	  	\chain\cons(\var, \stack, \genv) &  \val & \stempty &  \genvtwo
		& \tomachseathree &
		\chain &  \var & \stack &  \genv\cons\esub\var{\val}\cons\genvtwo
		\\

		 \chain & \var & \stack & \genv\cons\esub\var\val\cons\genvtwo
	  	&\tomachsub &
		 \chain & \renamenop\val & \stack & \genv\cons\esub\var\val\cons\genvtwo
	  	\\
	\end{array}}
\\[4pt]
\mbox{Where $\renamenop{\val}$ is any well-bound code $\alpha$-equivalent to $\val$ such that its }
\\ \mbox{bound names  are fresh with respect to those in the other data structures.}
\end{array}$
}
\caption{The Milner Abstract machine by Need (MAD).}
\label{fig:cbneed-machine}
\end{figure}

==> figures/figure-machine-gc.tex <==
% !TEX root = ../main.tex
\begin{figure}[t!]
\centering\small
%\fbox{
$\begin{array}{c}
\begin{array}{r@{\hspace{.25cm}} rcl  @{\hspace{.5cm}}  @{\hspace{.5cm}} r @{\hspace{.25cm}} rcl}
	\textsc{Roots} & \roots 	& \grameq & \set{\var_1,\ldots,\var_n} \ \ \ n\geq 0
	\\
	\textsc{States} &	\state	& \defeq & \fivestate\chain\tm\stack\env\roots
	&
	\textsc{Init.} &	\tm	& \compilrel{}{} & \fivestate\emptylist{\renamenop\tm}\emptylist\emptylist\emptyset
\end{array}
\\
%\hline

  	{\setlength{\arraycolsep}{0.3em}
  	\begin{array}{|c|c|c|c|c||l||c|c|c|c|c|ll}
	\hhline{-|-|-|-|-|-|-|-|-|-|-}
		 \mbox{Ch.} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} & \mbox{Roots} 
		&&
		 \mbox{Ch.} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} &  \mbox{Roots} \\
\hhline{=|=|=|=|=|=|=|=|=|=|=}
		 \multicolumn{4}{|c|}{\ldots} & \emptyset
	  	&\toecoseaone&
	  	 \multicolumn{4}{c|}{\ldots} & \emptyset
	  	\\
%\hhline{-|-|-|---|-|-|-}
%
		 \chain & \la\var\tm & \tmtwo \cons\stack  &\env & \emptyset
		& \toecobetaone &
		\chain &  \tm & \stack  &\esub\var\tmtwo\cons\env & \emptyset
		& \text{if }\var\in\fv\tm
		\\
		 \chain & \la\var\tm & \tmtwo \cons\stack  &\env & \emptyset
		& \toecobetatwo &
		\chain &  \tm & \stack  &\esub\var\tmtwo\cons\env & \set\var
		& \text{if }\var\notin\fv\tm
		\\
		
		 \multicolumn{4}{|c|}{\ldots} & \emptyset
	  	&\toecoseatwo &
		 \multicolumn{4}{c|}{\ldots}  & \emptyset
	  	\\
		
	  	\multicolumn{4}{|c|}{\ldots} & \emptyset
		& \toecoseathree &
		\multicolumn{4}{c|}{\ldots} & \emptyset
		\\
		
		\multicolumn{4}{|c|}{\ldots} & \emptyset
	  	&\toecosk &
		\multicolumn{4}{c|}{\ldots} & \emptyset
	  	\\
		
		\chain & \var & \stack & \env\cons\skesub\var\val\cons\envtwo & \emptyset
	  	&\toecossone &
		\chain & \renamenop{\val} & \stack & \env\cons\skesub\var\val\cons\envtwo  & \emptyset
		& \text{if }\var\in\fv{\chain,\stack,\env}
	  	\\
		
		\chain & \var & \stack & \env\cons\skesub\var\val\cons\envtwo & \emptyset
	  	&\toecosstwo &
		\chain & \val & \stack & \env\cons\envtwo & \emptyset
		& \text{if }\var\notin\fv{\chain,\stack,\env}
	  	\\
\hhline{-|-|-|-|-|-|-|-|-|-|-}
		\chain & \tm & \stack & \env\cons\semsub\var\tmtwo\cons\envtwo  & \set\var\uplus\roots
	  	&\toecogc &
		\chain & \tm & \stack & \env\cons\envtwo  & \rootstwo
		& (*)
	  	\\
\hhline{-|-|-|-|-|-|-|-|-|-|-}
	\end{array}}\\
	\mbox{(*) with }\rootstwo \defeq \roots \cup \set{\vartwo\in\fv{\tmtwo}\ |\ \env\cons\envtwo = \envthree\cons\semsub\vartwo\tmthree\cons\envfour\text{ and }\vartwo\notin\fv{\chain,\tm,\stack,\envthree}}
\end{array}$
%}
\caption{The Eagerly garbage COllecting Skeletal MAD (ECO Skeletal MAD).}
\label{fig:gc-machine}
\end{figure}

==> figures/figure-skeletal_machine.tex <==
% !TEX root = ../main.tex
\begin{figure}[t!]
\centering
\fbox{
\small
$\begin{array}{c}
\begin{array}{r@{\hspace{.5cm}} rcl  @{\hspace{1cm}} r @{\hspace{.5cm}} rcl}
	\textsc{Stacks} & \stack 	& \grameq & \stempty \mid \tm \cons \stack
	&
	\textsc{Chains} &	\chain	& \grameq & \stempty \mid \chain\cons(\var, \stack, \genv)
\\
       
\textsc{States} &	\state	& \defeq & \glamst\chain\tm\stack\genv
	&
	\textsc{Environments} & \genv	& \grameq & \stempty \mid \esub\var\tm \cons \genv \mid \skesub\var\val \cons \genv 	
\end{array}
\\[10pt]\hline

\textsc{Transitions}
\\
  	{\setlength{\arraycolsep}{0.35em}
  	\begin{array}{c|c|c|c||l||c|c|c|ccc}
		 \mbox{Chain} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} 
		&&
		 \mbox{Chain} &\mbox{Code} & \mbox{Stack} &  \mbox{Env} \\
\hhline{=|=|=|=|=|=|=|=|=}
		 \chain & \tm\tmtwo & \stack &  \genv
	  	&\tomachseaone&
	  	 \chain & \tm & \tmtwo\cons\stack & \genv
	  	\\

		 \chain & \la\var\tm & \tmtwo \cons\stack  &\genv
		& \tomachbeta &
		\chain &  \tm & \stack  &\esub\var\tmtwo\cons\genv
		\\

		 \chain & \var & \stack & \genv\cons\esub\var\tm\cons\genvtwo
	  	&\tomachseatwo &
		 \chain\cons(\var, \stack, \genv) & \tm & \stempty & \genvtwo
		 &\text{if }\tm\neq\val
	  	\\
		
	  	\chain\cons(\var, \stack, \genv) &  \val & \stempty &  \genvtwo
		& \tomachseathree &
		\chain &  \var & \stack &  \genv\cons\esub\var\val\cons\genvtwo
		\\

		 \chain & \var & \stack & \genv\cons\esub\var\val\cons\genvtwo
	  	&\tomachsk &
		 \chain & \var & \stack & \genv\cons\skesub\var{\val'}\cons\genvthree\cons\genvtwo
	  	\\
		
		 \chain & \var & \stack & \genv\cons\skesub\var\val\cons\genvtwo
	  	&\tomachhole{\sssym} &
		 \chain & \renamenop{\val} & \stack & \genv\cons\skesub\var\val\cons\genvtwo
	  	\\

	%  	(\genvthree, \var, \stack)\cons\chain & \vartwo & \stempty &  \genv\cons \skesub\vartwo\val \cons\genvtwo
	%	& \tomachseafour &
	%	\chain & \var & \stack & \genv\cons \skesub\var{\renamenop\val} \cons\genvthree\cons \skesub\vartwo\val \cons\genvtwo\\
	\end{array}}
\\[45pt]
\mbox{Where $\renamenop{\val}$ is any well-bound code $\alpha$-equivalent to $\val$ such that its bound names  }
\\ \mbox{are fresh with respect to those in the other data structures, and $(\valtwo,\genvthree) \defeq \splitfun{\discabs{\bmark\val}}$.}
\end{array}$
}
\caption{The Skeletal Milner Abstract machine by Need (Skeletal MAD).}
\label{fig:skeletal-machine}
\end{figure}

==> proofs/eco-implementation.tex <==
% !TEX root = ../main.tex
\begin{proof}
\applabel{thm:eco-implementation}\hfill
 \begin{enumerate}
 \item By induction on $\size{\run_{\ecosym}} \in \nat$. Cases:
  \begin{itemize}
  \item $\size{\run_{\ecosym}} = 0$. Then $\run_{\ecosym} \colon \compilreleco\tm\state \toeco^0 \state$ and hence there is an empty run $\run_{\symfont{S}}: \compilrel\tm\statethree \tosmad^0 \statethree$. By definition, $\state \defeq \fourstate\emptylist{\renamenop\tm}\emptylist\emptylist$ and $\statethree = \fivestate\emptylist{\renamenop\tm}\emptylist\emptylist\emptyset$ where the two $\renamenop\tm$ might have picked different renamings, let us note the resulting terms $\tm_1$ and $\tm_2$. Note that $\gcop\statethree = \fourstate\emptylist{\tm_2}\emptylist\emptylist \eqwbalpha  \fourstate\emptylist{\tm_1}\emptylist\emptylist=\state$, as required.
  
\item $\size{\run_{\ecosym}} > 0$. Then, $\run_{\ecosym} \colon \compilreleco\tm\state \toeco^* \statetwo$ is the concatenation of a run $\runtwo_{\symfont{S}} \colon \compilreleco\tm\state \toeco^* \statetwo$ followed by either:
\begin{enumerate}
\item \emph{No garbage}: a transition $\statetwo_\bullet \toeco \statetwo$ that is not a $\ecosym{\cdot}\beta_2$ nor a $\ecosym{\cdot}\gc$ transition;
\item \emph{Creation and elimination of garbage}: a run $\statetwo_\bullet \toecobetatwo\toecogc^* \statetwo$.
\end{enumerate}
By \ih applied to $\runtwo_{\ecosym}$, there exists a run $\runtwo_{\symfont{S}} \colon \statethree \tosmad^* \statefour_\bullet$ such that $\statetwo_\bullet \eqwbalpha\gcop{\statefour_\bullet}$. There are various cases:
\begin{enumerate}
\item \emph{No garbage 1}: $\statetwo_\bullet \toecop{a} \statetwo$ for $a\in{\seasym_1,\seasym_2,\seasym_3,\sksym}$. By strong bisimulation of $\eqwbalpha$ for the ECO Skeletal MAD (\reflemma{alpha-strong-bis}), $\gcop{\statetwo_\bullet} \toecop{a} \statetwo_\circ\eqwbalpha\statetwo$ for some $\statetwo_\circ$. In particular, $\gcop{\statetwo_\bullet}$ is not final. By the halt property (\refprop{eco-pseudo-distillery}.3), $\statefour_\bullet$ is not final, that is, $\statefour_\bullet \tosmad \statefour$. By inverse projection (\refprop{eco-pseudo-distillery}.1), that last transitions projects on the ECO machine. By determinism (\refprop{eco-pseudo-distillery}.2), the projected transition has to be $\gcop{\statetwo_\bullet} \toecop{a} \gcop\statefour=\statetwo_\circ$. Then $\statetwo_\bullet \tomachhole{a} \statefour$.

 Summing up, we built a run $\run_{\symfont{S}} \colon \statethree \tosmad^* \statefour_\bullet \tomachhole{a} \statefour$ such that $\gcop\statefour=\statetwo_\circ\eqwbalpha\statetwo$, as required.


\item \emph{No garbage 2}: $\statetwo_\bullet \toecobetaone \statetwo$ or $\statetwo_\bullet \toecossone \statetwo$. We reason as in the previous case, matching the transition with $\tomachbeta$ or $\tomachss$ on the Skeletal MAD.

\item \emph{No garbage 3}: $\statetwo_\bullet \toecosstwo \statetwo$. We reason as in case $a$, obtaining $\statetwo_\bullet \tomachss \statefour$, he only difference is that now the projected transition is $\gcop{\statetwo_\bullet} \toecosstwo \statetwo_\circ \eqwbalpha \gcop\statefour$. The statement still holds, as we obtain $\run_{\symfont{S}} \colon \statethree \tosmad^* \statefour_\bullet \tomachhole{a} \statefour$ with $\gcop\statefour\eqwbalpha\statetwo_\circ\eqwbalpha\statetwo$.



\item \emph{Creation and elimination of garbage}: $\statetwo_\bullet \toecobetatwo\toecogc^* \statetwo$. We reason as in case $a$, obtaining $\statetwo_\bullet \tomachbeta \statefour$ on the Skeletal MAD.
\end{enumerate}
 \end{itemize}

 %%%%%% Point 2
 \item By induction on $\size{\run_{\symfont{S}}} \in \nat$. Cases:
  \begin{itemize}
  \item $\size{\run_{\symfont{S}}} = 0$. Then $\run_{\symfont{S}}: \state \tosmad^0 \state$ with $\state \defeq \fourstate\emptylist{\renamenop\tm}\emptylist\emptylist$. Note that $\gcop\state \defeq \fivestate\emptylist{\renamenop\tm}\emptylist\emptylist\emptyset$ so that $\compilreleco\tm{\gcop\state}$ holds, and that obviously there is an empty run $\run_{\ecosym} \colon \gcop\state \toeco^0 \gcop\state$.
  
 \item  $\size{\run_{\symfont{S}}} > 0$. Then, $\run_{\symfont{S}} \colon \compilreleco\tm\state \tosmad^* \statetwo$ is the concatenation of a run $\runtwo_{\symfont{S}} \colon \compilreleco\tm\state \tosmad^* \statetwo_\bullet$ followed by a transition $\statetwo_\bullet \tosmad \statetwo$. By \ih applied to $\runtwo_{\symfont{S}}$, there exists a run $\derivtwo_{\ecosym} \colon \compilreleco\tm\gcop\state \toeco^* \eqwbalpha \gcop{\statetwo_\bullet}$. Cases of $\statetwo_\bullet \toeco \statetwo$:
\begin{enumerate}
\item \label{p:case-a}$\statetwo_\bullet \tomachhole{a} \statetwo$ for $a\in{\seasym_1,\seasym_2,\seasym_3,\sksym}$. By inverse projection (\refprop{eco-pseudo-distillery}.1.c), $\gcop{\statetwo_\bullet} \toecop{a} \gcop\statetwo$. Therefore, $\gcop\state \toeco^* \eqwbalpha \gcop{\statetwo_\bullet} \toecop{a} \gcop\statetwo$. Postponing $\eqwbalpha$ using \reflemma{alpha-strong-bis}, we obtain $\gcop\state \toeco^* \gcop{\statetwo_\bullet} \toecop{a} \eqwbalpha \gcop\statetwo$, as required.

\item $\statetwo_\bullet \tomachbeta \statetwo$. By inverse projection (\refprop{eco-pseudo-distillery}.1.a), we have either $\gcop{\statetwo_\bullet} \toecobetaone \gcop\statetwo$ or $\gcop{\statetwo_\bullet} \toecobetatwo \toecogc^* \gcop\statetwo$. In both cases, it goes as in case $a$.

\item $\statetwo_\bullet \tomachss \statetwo$. By inverse projection (\refprop{eco-pseudo-distillery}.1.b), we have either $\gcop{\statetwo_\bullet} \toecossone \gcop\statetwo$ or $\gcop{\statetwo_\bullet} \toecosstwo\statethree \eqwbalpha \gcop\statetwo$. In both cases, it goes as in case $a$.
\end{enumerate}
\end{itemize}
\item An immediate inspection of the proofs of the firs two points shows that the matching property holds.\qedhere
\end{enumerate}
\end{proof}

==> proofs/strong-bisimulation-proof-for-CBNeed.tex <==
% !TEX root = ../main.tex
Let $\tostructsym$ be the symmetric closure of the
union of the axiom defining $\eqstruct$.
Note that $\eqstruct$ is the reflexive--transitive closure of $\tostructsym$.
The proof is in two parts:
\begin{itemize}
\item[] (I) Prove the property holds for $\tostructsym$, \ie\
            if $\tm\towhl_{a}\tmtwo$ and $\tm\tostructsym\tmthree$, there exists $\tmfour$ s.t. $\tmthree\towhl_{a}\tmfour$ and $\tmtwo\eqstruct\tmfour$.
\item[] (II) Prove the property holds for $\eqstruct$ (\ie\ for many steps of $\tostructsym$) by resorting to (I).
\end{itemize}


The proof of (II) is immediate by induction on the number of $\tostructsym$ steps.
The proof of (I) goes by induction on the rewriting step $\togen$ (that, since $\togen$ is closed by evaluation contexts, becomes a proof by induction on the evaluation context $\evctx$). In principle, we should always consider the two directions of $\tostructsym$. Most of the time, however, one direction is obtained by simply reading the diagram of the other direction bottom-up, instead than top-down; these cases are simply omitted, we distinguish the two directions only when it is relevant.

\begin{enumerate}
\item \casealt{Base case 1: multiplicative root step $
            \tm = \sctxp{\l\var.\tmp}\tmfive
            \rtodb
            \tmtwo = \sctxp{\tmp\esub \var \tmfive}
            $}
Every application of $\eqstruct$ inside $\tmfive$ or inside one of the substitutions in $\sctx$ trivially commutes with the step. The interesting cases are those where structural equivalence has a critical pair with the step:
  \begin{enumerate}
\item \label{p:str-bis-need-base-db-apl}\caselight{Commutation with left of an application $\tostructapl$}.
		If $\sctx=\sctxtwo\esub\vartwo\tmfour$ then
		
		        $$\commutesdbEEABCD{\tostructapl}{=}{
            \sctxtwop{\l\var.\tmp}\esub\vartwo\tmfour\tmfive
        }{
            \sctxtwop{\tmp\esub\var\tmfive}\esub\vartwo\tmfour
        }{
            (\sctxtwop{\l\var.\tmp}\tmfive)\esub\vartwo\tmfour
        }{
            \sctxtwop{\tmp\esub\var\tmfive}\esub\vartwo\tmfour
        }
        $$

		
    % end dB vs apl

    % begin dB vs com
    \item \caselight{Commutation of independent substitutions $\tostructcom$}.
      The substitutions that are commuted by the $\tostructcom$ rule
      must be both in $\sctx$, \ie\ $\sctx$ must be of the form
      $\sctxtwop{\sctxthree\esub{\vartwo}{\tmthreep}\esub{\varthree}{\tmfourp}}$
      with $\varthree \not\in \fv{\tmthreep}$.
      Let $\sctxal = \sctxtwop{\sctxthree\esub{\varthree}{\tmfourp}\esub{\vartwo}{\tmthreep}}$.
      Then:
 \begin{center}
 \begin{tikzpicture}[ocenter]
  \node (s) {\normalsize$\sctxp{\l\var.\tmp}\tmtwop$};
  \node at (s.center)  [below =\nodeVerDist](s2) {\normalsize$\sctxpal{\l\var.\tmp}\tmtwop$};
  \node at (s2.center) [right= \nodeHorDist](t) {\normalsize$\sctxpal{\tmp\esub{\var}{\tmtwop}}$};
  \node at (s-|t) [](s1){\normalsize$\sctxp{\tmp\esub{\var}{\tmtwop}}$};
  \draw[->] (s) to node {\scriptsize $\db$} (s1);
  \node at \med{s.center}{s2.center}(eq1){\normalsize$\tostructcom$};
  \node at \med{s1.center}{t.center}(eq2){\normalsize$\tostructcom$};
\draw[->, dashed] (s2) to node {\scriptsize $\db$} (t);
\end{tikzpicture} 
\end{center}
    % end dB vs com

    % begin dB vs es
    \item \caselight{Composition of substitutions $\tostructes$}.
      The substitutions that appear in the left-hand side of the $\tostructes$ rule must both
      be in $\sctx$, \ie\ $\sctx$ must be of the form $\sctxtwop{\sctxthree\esub{\vartwo}{\tmthreep}\esub{\varthree}{\tmfourp}}$
      with $\varthree \not\in \fv{\sctxthreep{\l\var.\tmp}}$.
      Let $\sctxal = \sctxtwop{\sctxthree\esub{\vartwo}{\tmthreep\esub{\varthree}{\tmfourp}}}$. Exactly as in the previous case:
      \begin{center}
 \begin{tikzpicture}[ocenter]
  \node (s) {\normalsize$\sctxp{\l\var.\tmp}\tmtwop$};
  \node at (s.center)  [below =\nodeVerDist](s2) {\normalsize$\sctxpal{\l\var.\tmp}\tmtwop$};
  \node at (s2.center) [right= \nodeHorDist](t) {\normalsize$\sctxpal{\tmp\esub{\var}{\tmtwop}}$};
  \node at (s-|t) [](s1){\normalsize$\sctxp{\tmp\esub{\var}{\tmtwop}}$};
  \draw[->] (s) to node {\scriptsize $\db$} (s1);
  \node at \med{s.center}{s2.center}(eq1){\normalsize$\tostructes$};
  \node at \med{s1.center}{t.center}(eq2){\normalsize$\tostructes$};
\draw[->, dashed] (s2) to node {\scriptsize $\db$} (t);
\end{tikzpicture} 
\end{center}
  \end{enumerate}
%% end base multiplicative case


  \item \casealt{Base case 2: exponential root step $
            \tm = \evctxp{\var}\esub{\var}{\sctxp{\val}}
            \rtolsv
            \tmtwo = \sctxp{\evctxp{\val}\esub{\var}{\val}}
            $}
    Consider first the case when the $\tostructsym$-redex is internal
    to $\evctxp{\var}$. By \reflemma{cbneed_eqstruct_preserves_shapes}
    we know $\tostructsym$ preserves the shape of $\evctxp{\var}$,
    \ie\ $\evctxp{\var} \tostructsym \evctxpal{\var}$. Then:
    $$
    \commuteslsvEEABCD{\tostructsym}{\eqstruct}{
        \evctxp{\var}\esub{\var}{\sctxp{\val}}
    }{
        \sctxp{\evctxp{\val}\esub{\var}{\val}}
    }{
        \evctxpal{\var}\esub{\var}{\sctxp{\val}}
    }{
        \sctxp{\evctxpal{\val}\esub{\var}{\val}}
    }
    $$
    If the $\tostructsym$-redex is internal to one of the substitutions in $\sctx$, the proof is straightforward.
    Note that the $\tostructsym$-redex has always a substitution
    at the root. The remaining possibilities are that such
    substitution is in $\sctx$, or that it is precisely $\esub{\var}{\sctxp{\val}}$.
    Axiom by axiom:
    
    \begin{enumerate}

    % lsv vs. apl
    \item \label{p:str-bis-need-exp-apl}\caselight{Commutation with the left of an application $\tostructapl$}.
        The only possibility is that the substitution $\esub{\var}{\sctxp{\val}}$
        is commuted with the outermost application in $\evctxp{\var}$, \ie\ $\evctx = \evctxtwo\tmp$. The diagram is:
        
            $$
    \commuteslsvEEABCD{\tostructapl}{\tostructapl^*}{
        (\evctxtwop{\var}\,\tmp)\esub{\var}{\sctxp{\val}}
    }{
        \sctxp{(\evctxtwop{\val}\,\tmp)\esub{\var}{\val}}
    }{
        \evctxtwop{\var}\esub{\var}{\sctxp{\val}}\tmp
    }{
        \sctxp{\evctxtwop{\val}\esub{\var}{\val}}\,\tmp
    }
    $$

        
    
    % lsv vs. com
    \item \caselight{Commutation of independent substitutions $\tostructcom$}. Two sub-cases:
    \begin{enumerate}
        \item \label{p:str-bis-need-exp-com-one} \caselight{The commuted substitutions both belong to $\sctx$}. Let $\sctxal$ be the result of commuting them,
        and the diagram is:
                $$
        \commuteslsvEEABCD{\tostructcom}{\tostructcom}{
            \evctxp{\var}\esub{\var}{\sctxp{\val}}
        }{
            \sctxp{\evctxp{\val}\esub{\var}{\val}}
        }{
            \evctxp{\var}\esub{\var}{\sctxpal{\val}}
        }{
            \sctxpal{\evctxp{\val}\esub{\var}{\val}}
        }
        $$


        \item \label{p:str-bis-base-exp-com-two} \caselight{One of the commuted substitutions is $\esub{\var}{\sctxp{\val}}$}. Then
        $\evctx = \evctxtwo\esub{\vartwo}{\tmp}$ and $\esub{\var}{\sctxp{\val}}$ commutes with $\esub{\vartwo}{\tmp}$ (which implies $\var \not\in \fv{\tmp}$). Then:
        $$
        \commuteslsvEEABCD{\tostructcom}{\tostructcom^*}{
            \evctxtwop{\var}\esub{\vartwo}{\tmp}\esub{\var}{\sctxp{\val}}
        }{
            \sctxp{\evctxtwop{\val}\esub{\vartwo}{\tmp}\esub{\var}{\val}}
        }{
            \evctxtwop{\var}\esub{\var}{\sctxp{\val}}\esub{\vartwo}{\tmp}
        }{
            \sctxp{\evctxtwop{\val}\esub{\var}{\val}}\esub{\vartwo}{\tmp}
        }
        $$
\end{enumerate}
		%end of lsv vs. com

    % lsv vs. es
    \item \caselight{Composition of substitutions $\tostructes$}. Two sub-cases:
    \begin{enumerate}
        \item \caselight{The composed substitutions both belong to $\sctx$}. 
        Analogous to case \ref{p:str-bis-need-exp-com-one}.

				\item \label{p:str-bis-need-exp-comp-two}\caselight{One of the composed subtitutions is $\esub{\var}{\sctxp{\val}}$}.
        This is not possible if the rule is applied from left to right,
        since it would imply that
        $\evctxp\var = \evctxtwop\var\esub{\vartwo}{\tmp}$ with
        $\var \not\in \evctxtwop{\var}$, which is a contradiction.

        Finally, if the $\tostructes$ rule is applied from right to left,
        $\sctx$ is of the form $\sctxtwo\esub{\vartwo}{\tmp}$ and:
        $$
        \commuteslsvEEABCD{\tostructes}{=}{
            \evctxp{\var}\esub{\var}{\sctxtwop{\val}\esub{\vartwo}{\tmp}}
        }{
            \sctxtwop{\evctxp{\val}\esub{\var}{\val}}\esub{\vartwo}{\tmp}
        }{
            \evctxp{\var}\esub{\var}{\sctxtwop{\val}}\esub{\vartwo}{\tmp}
        }{
            \sctxtwop{\evctxp{\var}\esub{\var}{\val}}\esub{\vartwo}{\tmp}
        }
        $$
            \end{enumerate}
            % end of lsv vs. es
    \end{enumerate}
    % end of the base exponential case
  
\item \casealt{Inductive case 1: left of an application $\evctx = \evctxtwo\tmfive$}
  The situation is:
  $$\tm = \evctxtwop{\tmp}\,\tmfive \towhlcek \evctxtwop{\tmtwop}\,\tmfive = \tmtwo$$
  If the $\tostructsym$ step is internal to $\evctxtwop{\tmp}$, the result follows
  by \ih. The proof is also direct if $\tostructsym$ is internal to $\tmfive$.
  The nontrivial cases are those where $\tostructsym$ overlaps $\evctxtwop{\tmp}$ and $\tmfive$. The only possible case is that a substitution commutes with the topmost application via $\tostructapl$ (applied from right to left). There are two cases:
  \begin{enumerate}
  \item \caselight{The substitution comes from $\tmp$.}
        That is, $\evctxtwo = \ctxhole$ and $\tmp$ has a substitution at its root.
        Then $\tmp$ must be a $\rtolsv$-redex
        $\tmp = \evctxthreep{\var}\esub{\var}{\sctxp{\val}}$.
        We have:
        $$
        \commuteslsvEEABCD{\tostructapl}{\tostructapl^*}{
            \evctxthreep{\var}\esub{\var}{\sctxp{\val}}\,\tmfive
        }{
            \sctxp{\evctxthreep{\val}\esub{\var}{\val}}\,\tmfive
        }{
            (\evctxthreep{\var}\,\tmfive)\esub{\var}{\sctxp{\val}}
        }{
            \sctxp{(\evctxthreep{\val}\,\tmfive)\esub{\var}{\val}}
        }
        $$
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
  \item \label{p:str-bis-need-ind-leftap-apl-two}\caselight{The substitution comes from $\evctxtwo$.}
        That is: $\evctxtwo = \evctxthree\esub{\var}{\tmthreep}$.
        The proof is then straightforward:
        $$
        \commutesredEEABCD{\tostructapl}{\tostructapl}{
            \evctxthreep{\tmp}\esub{\var}{\tmthreep}\,\tmfive
        }{
            \evctxthreep{\tmtwop}\esub{\var}{\tmthreep}\,\tmfive
        }{
            (\evctxthreep{\tmp}\,\tmfive)\esub{\var}{\tmthreep}
        }{
            (\evctxthreep{\tmtwop}\,\tmfive)\esub{\var}{\tmthreep}
        }
        $$
  \end{enumerate}

\item \casealt{Inductive case 2: left of a substitution $\evctx = \evctxtwo\esub{\var}{\tmfive}$}
  The situation is:
  $$\tm = \evctxtwop{\tmp}\esub{\var}{\tmfive} \towhlcek \evctxtwop{\tmtwop}\esub{\var}{\tmfive} = \tmtwo$$
  If the $\tostructsym$ step is internal to $\evctxtwop{\tmp}$,
  the result follows by \ih. If it is internal to $\tmfive$, the steps are
  orthogonal, which makes the diagram trivial.
  The remaining possibility is that the substitution $\esub{\var}{\tmfive}$
  is involved in the $\tostructsym$ redex.
  By case analysis on the kind of the step $\eqstruct_b$:
  \begin{enumerate}
  \item \caselight{Commutation with the left of an application $\tostructapl$}.
    $\evctxtwop{\tmp}$ must be an application. Two
    possibilities:
    \begin{enumerate}
    \item \caselight{The application comes from $\tmp$.}
          That is, $\evctxtwo = \ctxhole$ and $\tmp$ is a $\rtodb$-redex
          $\tmp = \sctxp{\l\vartwo.\tmpp}\,\tmfour$. This is exactly as the base case \ref{p:str-bis-need-base-db-apl} (read bottom-up).

    \item \caselight{The application comes from $\evctxtwo$, \ie\ $\evctxtwo = \evctxthree\,\tmthreep$}. This is exactly as the inductive case \ref{p:str-bis-need-ind-leftap-apl-two} (read bottom-up).
    \end{enumerate}

  \item \caselight{Commutation of independent substitutions $\tostructcom$}.
	Since $\evctxtwop{\tmp}$ must have a substitution at the root,
    there are two possibilities:
    \begin{enumerate}
    \item \caselight{The substitution comes from $\tmp$.}
          That is, $\evctxtwo = \ctxhole$ and $\tmp$ is a $\rtolsv$-redex
          $\tmp = \evctxthreep{\vartwo}\esub{\vartwo}{\sctxp{\val}}$,
          with $\var \not\in \fv{\sctxp{\val}}$. This case is exactly as the base exponential case \ref{p:str-bis-base-exp-com-two} (read bottom-up).
    \item \caselight{The substitution comes from $\evctxtwo$.}
		That is, $\evctxtwo = \evctxthree\esub{\vartwo}{\tmthreep}$
		with $\var \not\in \fv{\tmthreep}$. The diagram is:
          $$
          \commuteslsvEEABCD{\tostructcom}{\tostructcom}{
			\evctxthreep{\tmp}\esub{\vartwo}{\tmthreep}\esub{\var}{\tmfive}
          }{
			\evctxthreep{\tmtwop}\esub{\vartwo}{\tmthreep}\esub{\var}{\tmfive}
          }{
			\evctxthreep{\tmp}\esub{\var}{\tmfive}\esub{\vartwo}{\tmthreep}
          }{
			\evctxthreep{\tmtwop}\esub{\var}{\tmfive}\esub{\vartwo}{\tmthreep}
          }
          $$
    \end{enumerate}
  \item \caselight{Composition of substitutions $\tostructes$}.
	As in the previous case, there are two possibilities:
    \begin{enumerate}
    \item \caselight{The substitution comes from $\tmp$.}
          That is, $\evctxtwo = \ctxhole$ and $\tmp$ is a $\rtolsv$-redex
          $\tmp = \evctxthreep{\vartwo}\esub{\vartwo}{\sctxp{\val}}$,
          with $\var \not\in \fv{\evctxthreep{\vartwo}}$. 
          This case is exactly as the base exponential case \ref{p:str-bis-need-exp-comp-two} (read bottom-up).

    \item \caselight{The substitution comes from $\evctxtwo$.}
		That is, $\evctxtwo = \evctxthree\esub{\vartwo}{\tmthreep}$
		with $\var \not\in \fv{\evctxthreep{\tmp}}$. The diagram is:
          $$
          \commutesredEEABCD{\tostructes}{\tostructes}{
			\evctxthreep{\tmp}\esub{\vartwo}{\tmthreep}\esub{\var}{\tmfive}
          }{
			\evctxthreep{\tmtwop}\esub{\vartwo}{\tmthreep}\esub{\var}{\tmfive}
          }{
			\evctxthreep{\tmp}\esub{\vartwo}{\tmthreep\esub{\var}{\tmfive}}
          }{
			\evctxthreep{\tmtwop}\esub{\vartwo}{\tmthreep\esub{\var}{\tmfive}}
          }
          $$
	\end{enumerate}
	% end of left-of-sub vs. comp
	
  \end{enumerate}
  % end of left-of-sub
  
  \item \casealt{Inductive case 3: inside a hereditary head substitution $\evctx = \evctxtwop\var\esub{\var}{\evctxthree}$}
  The situation is:
  $$\tm = \evctxtwop\var\esub{\var}{\evctxthreep\tmfive} \togen \evctxtwop\var\esub{\var}{\evctxthreep\tmfivep} = \tmtwo$$
  If $\tostructsym$ is internal to $\evctxtwop\var$ the two steps clearly commutes. If $\tostructsym$ is internal to $\evctxthreep\tmfive$ we conclude using the \ih. The remaining cases are when $\tostructsym$ overlaps with the topmost constructor. Axiom by axiom:
  \begin{enumerate}
  \item \caselight{Commutation with the left of an application $\tostructapl$}. It must be that $\evctxtwop\var=\evctx''''\ctxholep\var\tmfour$ with $\var\notin\fv\tmfour$. Then  the two steps simply commute:
          $$
        \commutesredEEABCD{\tostructapl}{\tostructapl}{
            (\evctx''''\ctxholep\var\tmfour)\esub{\var}{\evctxthreep\tmfive}
        }{
            (\evctx''''\ctxholep\var\tmfour)\esub{\var}{\evctxthreep\tmfivep}
        }{
            \evctx''''\ctxholep\var\esub{\var}{\evctxthreep\tmfive}\tmfour
        }{
            \evctx''''\ctxholep\var\esub{\var}{\evctxthreep\tmfivep}\tmfour
        }
        $$

  \item \caselight{Commutation of independent substitutions $\tostructcom$}. It must be that $\evctxtwop\var=\evctx''''\ctxholep\var\esub\vartwo\tmfour$ with $\var\notin\fv\tmfour$. Then the two steps simply commute:
          $$
        \commutesredEEABCD{\tostructapl}{\tostructapl}{
            \evctx''''\ctxholep\var\esub\vartwo\tmfour\esub{\var}{\evctxthreep\tmfive}
        }{
            \tm_1
        }{
            \tm_2
        }{
            \tm_3
        }
        $$
        where
        \begin{align*}
        	\tm_1 := \evctx''''\ctxholep\var\esub\vartwo\tmfour\esub{\var}{\evctxthreep\tmfivep},\\
        	\tm_2 := \evctx''''\ctxholep\var\esub{\var}{\evctxthreep\tmfive}\esub\vartwo\tmfour,\\
        	\tm_3 := \evctx''''\ctxholep\var\esub{\var}{\evctxthreep\tmfivep}\esub\vartwo\tmfour.
        \end{align*}

  \item \caselight{Composition of substitutions $\tostructes$}. There are various sub-cases
    \begin{enumerate}
    	\item \caselight{$\esub{\var}{\evctxthreep\tmfive}$ enters in a substitution}. It must be that $\evctxtwop\var=\evctx_1\ctxholep\vartwo\esub\vartwo{\evctx_2\ctxholep\var}$ with $\var\notin\fv{\evctx_1\ctxholep\vartwo}$. Then the diagram is:
	        $$
        \commutesredEEABCD{\tostructes}{\tostructes}{
            \evctx_1\ctxholep\vartwo\esub\vartwo{\evctx_2\ctxholep\var}\esub{\var}{\evctxthreep\tmfive}
        }{
            \tm_1
        }{
            \tm_2
        }{
            \tm_3
        }
        $$
        \begin{align*}
        	\tm_1 &:= \evctx_1\ctxholep\vartwo\esub\vartwo{\evctx_2\ctxholep\var}\esub{\var}{\evctxthreep\tmfivep},\\
        	\tm_2 &:= \evctx_1\ctxholep\vartwo\esub\vartwo{\evctx_2\ctxholep\var\esub{\var}{\evctxthreep\tmfive}},\\
        	\tm_3 &:= \evctx_1\ctxholep\vartwo\esub\vartwo{\evctx_2\ctxholep\var\esub{\var}{\evctxthreep\tmfivep}}.
        \end{align*}

	
			\item \caselight{a substitution pops out of $\esub{\var}{\evctxthreep\tmfive}$}. Two sub-cases:
			\begin{enumerate}
				\item \caselight{The substitution comes from $\evctxthree$}. Then $\evctxthreep\tmfive=\evctx''''\ctxholep\tmfive\esub\vartwo\tmfour$. The diagram is:
				$$\commutesredEEABCD{\tostructes}{\tostructes}{
            \evctxtwop\var\esub{\var}{\evctx''''\ctxholep\tmfive\esub\vartwo\tmfour}
        }{
            \tm_1            
        }{
            \tm_2
        }{
            \tm_3
        }$$
        where
        \begin{align}
        	\tm_1 &:= \evctxtwop\var\esub{\var}{\evctx''''\ctxholep\tmfivep\esub\vartwo\tmfour},\\
        	\tm_2 &:= \evctxtwop\var\esub{\var}{\evctx''''\ctxholep\tmfive}\esub\vartwo\tmfour,\\
        	\tm_3 &:= \evctxtwop\var\esub{\var}{\evctx''''\ctxholep\tmfivep}\esub\vartwo\tmfour.
        \end{align}

        
				\item \caselight{The substitution comes from $\tmfive$}. Then $\evctxthree=\ctxhole$ and $\tmfive$ is a $\rtolsv$-redex
          $\tmp = \evctx''''\ctxholep\vartwo\esub{\vartwo}{\sctxp{\val}}$ and the diagram is:
   $$\commuteslsvEEABCD{\tostructes}{\tostructes^*}{
            \evctxtwop\var\esub{\var}{ \evctx''''\ctxholep\vartwo\esub{\vartwo}{\sctxp{\val}} }
        }{
            \tm_1            
        }{
            \tm_2
        }{
            \tm_3
        }$$
        where
        \begin{align}
        	\tm_1 &:= \evctxtwop\var\esub{\var}{ \sctxp{\evctx''''\ctxholep\val\esub{\vartwo}{\val}}},\\
        	\tm_2 &:= \evctxtwop\var\esub{\var}{ \evctx''''\ctxholep\vartwo}\esub{\vartwo}{\sctxp{\val}},\\
        	\tm_3 &:= \sctxp{\evctxtwop\var\esub{\var}{ \evctx''''\ctxholep\val}\esub{\vartwo}{\val}}.
        \end{align}
  		\end{enumerate}
		\qed
  	\end{enumerate}
  \end{enumerate}
\end{enumerate}


